Local well-posedness for dispersive equations with bounded data

Given sufficiently regular data \textit{without} decay assumptions at infinity, we prove local well-posedness for non-linear dispersive equations of the form \[ \partial_t u + \mathsf A(\nabla) u + \mathcal Q(|u|^2) \cdot \nabla u= \mathcal N (u, \overline u), \] where $\mathsf A(\nabla)$ is a Fourier multiplier with purely imaginary symbol of order $\sigma + 1$ for $\sigma > 0$, and polynomial-type non-linearities $\mathcal Q(|u|^2)$ and $\mathcal N(u, \overline u)$. Our approach revisits the classical energy method by applying it within a class of local Sobolev-type spaces $\ell^\infty_{\mathsf A(\xi)} H^s (\mathbb R^d)$ which are adapted to the dispersion relation in the sense that functions $u$ localised to dyadic frequency $|\xi| \approx N$ have size \[ ||u||_{\ell^\infty_{\mathsf A(\xi)} H^s} \approx N^s \sup_{{\operatorname{diam}(Q) = N^\sigma}} ||u||_{L^2_x (Q)}. \] In analogy with the classical $H^s$-theory, we prove $\ell^\infty_{\mathsf A(\xi)} H^s$-local well-posedness for $s > \tfrac{d}2 + 1$ for the derivative non-linear equation, and $s > \tfrac{d}2$ without the derivative non-linearity. As an application, we show that if in addition the initial data is spatially almost periodic, then the solution is also spatially almost periodic.

==> internal/gwp.tex <==
We consider the defocusing non-linear Schrodinger equation with smooth power-type non-linearity 
    \begin{equation}
        \partial_t u + i \partial_x^2 u =  i |u|^{p - 1} u. 
    \end{equation}
Conservation of mass 
    \[
        M[u] 
            := \int_\R |u|^2 \, dx, 
    \]
and Hamiltonian,
    \[
        E[u] 
            := \int_\R \frac12 |\partial_x u|^2 + \frac1p |u|^p \, dx . 
    \]
Define the local mass 
    \[
        M_R[u] := \sup_{y \in \R} \int_\R \chi \big( \tfrac{x - y}{R} \big) |u|^2 \, dx.  
    \] 
Then differentiating  
    \begin{align*}
        \frac{d}{dt}\int_\R \chi \big( \tfrac{x - y}{R} \big) |u|^2 \, dx
            &= \Re \int_\R \chi \big( \tfrac{x - y}{R} \big) \overline u \partial_t u \, dx \\
            &= \Re \int_\R \chi \big( \tfrac{x - y}{R} \big) \overline u \big(i \partial_x^2 u + i |u|^{p - 1} u \big) \,dx \\
            &= \Re \int_\R \chi \big( \tfrac{x - y}{R} \big) \big(- i |\partial_x u|^2 + i |u|^p \big)\, dx - \frac1R \Re \int_\R  \chi' \big( \tfrac{x - y}{R} \big) (i \overline u \partial_x u) \, dx \\
            &= - \frac1R \Re \int_\R  \chi' \big( \tfrac{x - y}{R} \big) (i \overline u \partial_x u) \, dx. 
    \end{align*}
We can therefore estimate the mass by 
    \[
        \left|\frac{d}{dt}\int_\R \chi \big( \tfrac{x - y}{R} \big) |u|^2 \right|       
            \lesssim \frac1R M_R[u]^{1/2} E_R [u]^{1/2}. 
    \]    
To control the energy
    \begin{align*}
        \frac{d}{dt} \int_\R \chi \big( \tfrac{x - y}{R} \big) \Big( \frac12 |\partial_x u|^2 + \frac1p |u|^p \Big) \, dx 
            &= \Re \int_\R \chi \big( \tfrac{x - y}{R} \big) \Big( \overline{\partial_x u} \partial_x \partial_t u + |u|^{p - 1} \overline u \partial_t u \Big) \, dx \\
            &= \Re \int_\R \chi \big( \tfrac{x - y}{R} \big)\overline{\Big( - {\partial_x^2 u} + |u|^{p - 1}  u\Big)}\partial_t u \, dx - \frac1R \Re \int_\R \chi' \big( \tfrac{x - y}{R} \big) \big(\overline{\partial_x u} \partial_t u\big)\, dx \\
            &= \Re \int_\R \chi \big( \tfrac{x - y}{R} \big) i{\Big| - {\partial_x^2 u} + |u|^{p - 1}  u\Big|^2} \, dx - \frac1R \Re \int_\R \chi' \big( \tfrac{x - y}{R} \big) \big(\overline{\partial_x u} \partial_t u\big)\, dx\\
            &= \frac1R \Re \int_\R \chi' \big( \tfrac{x - y}{R} \big) \overline{\partial_x u} \Big( i \partial_x^2 u + |u|^{p - 1} u \Big)\, dx. 
    \end{align*}    
By Sobolev embedding, Cauchy-Schwartz, Sobolev embedding, and the energy estimate, 
    \begin{align*}
        \Big| \frac1R \int_\R \chi' \big( \tfrac{x - y}{R} \big) \overline{\partial_x u}  \partial_x^2 u \, dx \Big|
            &\lesssim \frac{1}{R^{1/2}} \left( \int_\R \chi' \big( \tfrac{x - y}{R} \big) |\partial_x u|^2\right)^{1/2} ||\partial_x^2 u||_{L^\infty} \\
            &\lesssim \frac{1}{R^{1/2}} E_R[u]^{1/2} ||u||_{\ell^\infty H^s} \\
            &\lesssim \frac{1}{R^{1/2}} E_R[u]^{1/2} ||u_0||_{\ell^\infty H^s} \exp \Big( \int_0^t C ||u(t')||_{L^\infty_x}^{p - 1} dt'\Big)\\
            &\lesssim \frac{1}{R^{1/2}} E_R[u]^{1/2} ||u_0||_{\ell^\infty H^s} \exp \Big( \int_0^t C (M_R[u]^{1/2} + E_R[u]^{1/2})^{p - 1} dt'\Big)
    \end{align*}
and by Cauchy-Schwartz
    \begin{align*}
        \Big| \frac1R \int_\R \chi' \big( \tfrac{x - y}{R} \big) \overline{\partial_x u}  |u|^{p - 1} u \, dx \Big|
            &\lesssim \frac1R E_R[u]. 
    \end{align*}
We are now ready to run a bootstrap argument. By Cauchy-Schwartz, 
    \[
        M_R [u_0] + E_R [u_0] \leq R (||u_0||_{L^\infty_x}^2 + ||\partial_x u_0||_{L^\infty_x}^2 + ||u_0||_{L^\infty_x}^p) \leq CR
     \] 
Let's suppress the dependence on the initial data in the constant $C$. Making the bootstrap assumption that $[0, T]$ is an interval for which $M_R[u] + E_R[u] \leq 2C R$, then integrating the differential inequalities,
    \begin{align*}
        M_R [u(t)] + E_R[u(t)]
            &\leq M_R [u_0] + E_R [u_0] \\
            &\qquad + \int_0^t O\Big( \frac1R M_R[u]^{1/2} E_R[u]^{1/2} + \frac{1}{R^{1/2}} E_R[u]^{1/2} ||u_0||_{\ell^\infty H^s} \exp(T R^{O(1)}) + \frac1R E_R[u]\Big) \, dx\\
            &\leq CR + O \Big( T + T \exp(T R^{O(1)}) \Big)\\
            &\leq \frac32 CR 
    \end{align*}
after taking $T$ growing sufficiently slowly in $R$. 

The exponential is not favourable for closing the bootstrap for large $T$... need to work smarter than just energy estimate for controlling $||\partial_x^2 u||$. 

 Goal: control growth of $||\partial_x^2 u||_{L^\infty}$ so that grows slower than energy.
